GSMFlow: Generation Shifts Mitigating Flow for Generalized Zero-Shot Learning

Generalized Zero-Shot Learning (GZSL) aims to recognize images from both the seen and unseen classes by transferring semantic knowledge from seen to unseen classes. It is a promising solution to take the advantage of generative models to hallucinate realistic unseen samples based on the knowledge learned from the seen classes. However, due to the generation shifts, the synthesized samples by most existing methods may drift from the real distribution of the unseen data. To address this issue, we propose a novel flow-based generative framework that consists of multiple conditional affine coupling layers for learning unseen data generation. Specifically, we discover and address three potential problems that trigger the generation shifts, i.e., semantic inconsistency, variance collapse, and structure disorder. First, to enhance the reflection of the semantic information in the generated samples, we explicitly embed the semantic information into the transformation in each conditional affine coupling layer. Second, to recover the intrinsic variance of the real unseen features, we introduce a boundary sample mining strategy with entropy maximization to discover more difficult visual variants of semantic prototypes and hereby adjust the decision boundary of the classifiers. Third, a relative positioning strategy is proposed to revise the attribute embeddings, guiding them to fully preserve the inter-class geometric structure and further avoid structure disorder in the semantic space. Extensive experimental results on four GZSL benchmark datasets demonstrate that GSMFlow achieves the state-of-the-art performance on GZSL.

==> files/sections/approach.tex <==
This section begins with formulating the GZSL problem and introducing the notations. The proposed GSMFlow is outlined next, followed by the visual perturbation strategy and the relative positioning approach to mitigate the generation shifts problem. The model training and zero-shot recognition are introduced lastly.



% \subsection{Overall Idea}
% In this paper, we leverage a conditional generative flow to generate fake visual features for unseen samples. 
% \noindent \textbf{Distribution Collapse Problem:} A common problem existing in generative methods that jeopardises the GZSL performance is that the generated unseen distributions are usually collapsed into fixed modes. The cause of this problem is a result of domain shift \cite{fu2015transductive}. It refers to the phenomenon that although some classes share the same attributes, their visual appearances are reflected differently, \textit{e.g.,} the `hasTail' attribute reflects different styles for `pig' and `horse'. Thus, learning the visual appearance on seen classes may not be able to generalize on unseen classes. 

% To alleviate this problem, we propose a visual perturbation strategy to encourage diverse sample generation on unseen classes. 

\subsection{Preliminaries}
Consider two datasets - a seen set $\mathcal{S}$ and an unseen set $\mathcal{U}$. The seen set $\mathcal{S}$ contains $N^s$ training samples $\vx^s \in \mathcal{X}$ and the corresponding class labels $\vy^s$, \textit{i.e.}, $\mathcal{S} = \{ \vx_{(i)}^{s}, \vy_{(i)}^{s} \}_{i=1}^{N^s}$. Similarly, $\mathcal{U} = \{ \vx_{(i)}^{u}, \vy_{(i)}^{u} \}_{i=1}^{N^u}$, where $N^u$ is the number of unseen samples. There are $C_s$ seen and $C_u$ unseen classes, so that $\vy^s \in \{1,\ldots,C_s \}$ and $\vy^u \in \{C_s+1,\ldots,C_u\}$. Note that the seen and unseen classes are mutually exclusive. There are $C_s+C_u$ class-level semantic vectors $\va \in \mathcal{A}$, where the class-level semantic vectors for the seen and unseen classes are $\{\va_{i}^{s}\}_{i=1}^{C_s}$ and $\{\va_{i}^{u}\}_{i=1}^{C_u}$, respectively.
$\va_{i}$ represents the semantic vector for the $i$-th class. In the setting of GZSL, we only have access to the seen samples $\mathcal{S}$ and semantic vectors $\{\va_{i}^{s}\}_{i=1}^{C_s}$ during training. Hence, for brevity, in the demonstration of the training process, we will omit the superscript $s$ for all the seen samples, \textit{i.e.}, $\vx=\vx^s$, $\va = \va^s$.

\subsection{Conditional Generative Flow}
To model the distribution of unseen visual features, we resort to conditional generative flows \cite{ardizzone2019guided}, a stream of simple yet powerful generative models. 

A conditional generative flow learns inference and generation within the same network. Let $\vz \in \mathcal{Z}$ be a random variable from a particular prior distribution $p_{Z}$, \textit{e.g.,} Gaussian, which has the same dimension as the visual features. We denote the inference process as the forward transformation $f(\cdot): \mathcal{X} \times \mathcal{A} \rightarrow \mathcal{Z}$, whose inverse transformation $g(\cdot) = f^{-1}(\cdot) : \mathcal{Z} \times \mathcal{A} \rightarrow \mathcal{X}$ is the generation process. The transformation is composed of $L$ bijective transformations $f(\cdot) = f_1(\cdot) \circ f_2(\cdot) \circ... \circ f_L(\cdot)$, the forward and inverse computations are the composition of the $L$ bijective transformations. 
Then, we can formalize the \textit{conditional generative flow} as:
\begin{equation}
\begin{gathered}
  \vz = f(\vx ; \va, \theta), \quad\vz \sim  \mathcal{N}(\bm{0}, \bm{I}),
\end{gathered}
\end{equation}
where the transformation $f(\cdot)$ parameterized with $\theta$ learns to transform a sample $\vx$ in the target distribution to the prior data distribution $p_Z$ conditioned on the corresponding class-level semantic vector $\va$. The forward transformation $g(\cdot)$ has its inverse transformation $g(\cdot) = f^{-1}(\cdot)$, which flows from the prior distribution $p_Z$ towards the target data distribution $p_X$:
\begin{equation}
\begin{gathered}
  \vx = g(\vz; \va, \theta).
\end{gathered}
\end{equation}
With the \textit{change of variable formula}, the bijective function $f(\cdot)$ can be trained through maximum log-likelihood:
\begin{equation}
\begin{gathered}
  \log p_{X}(\vx;\va, \theta) =\log p_{Z}(f(\vx;\va, \theta)) + \log\Big\lvert \text{det}(\frac{\partial f}{\partial \vx} ) \Big\rvert,
\end{gathered}
\end{equation}
where the latter half term denotes the logarithm of the determinant of the Jacobian matrix.

According to Bayes' theorem, the posterior distribution $p_{X}(\theta ; \vx,\va)$ for the parameter $\theta$ is proportional to $p_{X}(\vx;\va,\theta) p_{\theta}(\theta)$. The objective function can then be formulated as:
\begin{equation}
\begin{gathered}
  \mathcal{L}_{flow} = \mathbb{E}[-\log p_{X}(\vx;\va,\theta)] - \log p_{\theta}(\theta),
  \label{flow}
\end{gathered}
\end{equation}

\begin{figure}[t]
\centering
\includegraphics[width=85mm]{files/graphics/coupling.pdf}
\caption{The flowcharts of the conditional affine coupling layers. (a) The transformation flowchart when training the model. (b) The inverse direction for generating new samples.}
\label{coupling}
\end{figure}

% The generative flow is composed of $L$ bijective transformations $f(\cdot) = f_{L}(\cdot)\circ ... \circ f_2(\cdot) \circ f_1(\cdot)$.
% The Coupling flow, as the most widely used flow architecture, is adopted to enable highly expressive transformations.
% Let $g_1(\cdot),...,g_L(\cdot)$ be a set of L bijective transformations and  $g(\cdot) = g_{L}(\cdot)\circ ... \circ g_2(\cdot) \circ g_1(\cdot)$ is the composition of the transformations. Thus, the inverse function $f(\cdot)$ can be:
% \begin{equation}
% \begin{gathered}
% f(\cdot) = f_{1}(\cdot)\circ ... \circ f_{L-1}(\cdot) \circ f_L(\cdot).
% \end{gathered}
% \end{equation}
The composed bijective transformations are $L$ conditional affine coupling layers. As shown in Figure \ref{coupling}, in the forward transformation, each layer splits the input vector $\vu$ into two factors $[\vu_1, \vu_2]$. Note that in the first coupling layer, the input is $\vx$. Within each coupling layer, the internal functions $\vs_1(\cdot)$, $\vs_2(\cdot)$, and $\vt_1(\cdot)$, $\vt_2(\cdot)$ are formulated as:
\begin{equation}
\begin{gathered}
  \vv_1 = \vu_1 \odot \text{exp}\big(s_1([\vu_2,\va])\big) + t_1([\vu_2,\va]), \\
  \vv_2 = \vu_2 \odot \text{exp}\big(s_2([\vv_1,\va])\big) + t_2([\vv_1,\va]),
\end{gathered}
\end{equation}
where $\odot$ is the element-wise multiplication and the outputs $\vv_1$ and $\vv_2$ are fed into the next affine transformation.  In the last coupling layer, the output will be $\vz$. In the inverse direction, the conditional affine coupling module takes $\vv_1$ and $\vv_2$ as inputs:
\begin{equation}
    \begin{split}
    &\vu_2 = \big(\vv_2 - t_2([\vv_1,\va])\big) \oslash \text{exp}\big(s_2([\vv_1,\va])\big), \\
    &\vu_1 = \big(\vv_1 - t_1([\vu_2,\va])\big) \oslash \text{exp}\big(s_1([\vu_2,\va])\big),
    \end{split}
\end{equation}
where $\oslash$ is the element-wise division. \noindent As proposed in Real NVP \cite{dinh2016density}, when combining coupling layers, the Jacobian determinant remains tractable and its logarithm is the sum of $s_1(\cdot)$ and $s_2(\cdot)$ over visual feature dimensions.


\noindent \textbf{Discussion: Comparison to IZF.} 
Comparing to state-of-the-art approach IZF \cite{shen2020invertible} that also leverages a conditional generative flow in GZSL, our proposed GSMFlow differs in two aspects: 

1) \textit{Explicit conditional encoding.} In the training stage, IZF learns conditional encoding by disentangling the visual features into semantic and non-semantic vectors:
\begin{equation}
\begin{gathered}
  \text{[}\vz,\va \text{]} = f(\vx, \theta).
\end{gathered}
\end{equation} 
We argue that this approach of incorporating conditional information is implicit and may cause the generated samples to be incoherent with the given attributes and deviated from the real distribution. Instead, we explicitly blend the semantic information into each of the bijective coupling layers. By repeatedly enhancing the impact of the semantic information in the model, the generated visual samples tend to be more semantically consistent.

2) \textit{Drawbacks of the negative MMD.} In IZF, a negative Maximum Mean Discrepancy (MMD) regularization is applied to increase the discrepancy between the generated unseen distributions and the real distributions of the seen classes. We argue that this regularization is infeasible for the two mixed distributions of seen and unseen classes. MMD is commonly used in the domain adaptation that minimizes the discrepancy between the source and the target domains. However, in GZSL, as the seen and unseen classes generally come from the same domain, their visual relationships are highly coalesced. Hence, generally separating the two distributions may cause unexpected distribution shifts, which is undesirable for generating realistic unseen samples. 

In addition to the above differences, we also identify two problems, \textit{i.e.,} variance collapse and structure disorder. Accordingly, the visual perturbation and the relation positioning strategies are proposed to handle the two problems.

% investigate to preserve the intra-class variance and enhance the inter-class relationship.
% Generative zero-shot learning (GenZSL) based on conditional generative flows has been investigated in IZF \cite{shen2020invertible}. The way how IZF handles conditional information considerably differs from our approach. In our method, affine coupling functions learn by progressively adding semantic information to each coupling function, while they require the forward function $f(\vx,\theta)$ to output both $\vz$ and $\va$, such that:
% \begin{equation}
% \begin{gathered}
%   \text{[}\vz,\va \text{]} = f(\vx, \theta),
% \end{gathered}
% \end{equation}
% where the semantic vectors can be yielded in the inverse function $f(\cdot)$, but this is unnecessary in GZSL task. As there is no constraint in the intermediate affine coupling layers, directly encouraging the independence between $\vz$ and $\va$ in the final output can potentially degenerate the generalization power of forward function $g(\cdot)$ to unseen classes, which is experimentally investigated in the Experiments Section 4.4. As such, we claim that our design choice, which inserts the semantic vectors into each affine coupling layer, is easier to train and recursively enhances the conditional information.

% Also, IZF leverages a negative MMD regularization to increase the divergence between the generated distributions of seen and unseen classes in the visual space. 
% Minimizing a positive MMD 
% A positive MMD can directly minimize the divergence between two distributions. However, in the inductive setting of GZSL, the visual features of unseen classes are unavailable. Thus, it is implicit to measure how far the negative MMD should separate the seen and unseen classes. Further, generally increasing the divergence between the seen and unseen classes may jeopardise the generalization ability to unseen classes.
% However, unlike the positive MMD that directly minimizing the divergence between two distributions, it is implicit to measure how far the negative MMD should separate the seen and unseen classes without knowing the real distribution of unseen classes in the inductive setting of ZSL.

% it is implicit to measure how far the negative MMD should separate the seen and unseen classes. 
% Without knowing the real distribution of unseen classes, we can hardly know how far should we push unseen classes away. Further, generally increasing the divergence between seen and unseen classes may jeopardise the generalization ability to unseen classes. 

\subsection{Visual Perturbation}
To mitigate the variance collapse problem, we introduce a simple yet effective visual perturbation strategy to preserve the intra-class variance. We begin with sampling a perturbation vector $\ve \in \mathbb{R}^{d_v}$ from Gaussian distribution with the same size $d_v$ as the visual features:
\begin{equation}
\begin{gathered}
  \ve \sim \mathcal{N}(\bm{0},\bm{I}).
\end{gathered}
\end{equation}
In the high-dimensional visual space, we aim to make the perturbation more diverse. Hence, we construct a dropout mask $\vm$ to selectively filter out some of the dimensions of the perturbation vectors:
\begin{equation}
\begin{gathered}
  \vm_j = \begin{cases}
\bm{1}, \quad \text{with}~ p_{drop}
\\
\bm{0}, \quad \text{otherwise}
\end{cases}
\end{gathered}
\end{equation}
where $p_{drop}$ is the probability of keeping the perturbation in the $j$-th dimension. Then, we have the perturbation vector after applying the dropout map:
\begin{equation}
\begin{gathered}
\hat{\ve} = \ve \cdot \vm.
\end{gathered}
\end{equation}
\noindent A virtual sample $\vx^{vir}$ can be then yielded by:
\begin{equation}
\begin{gathered}
  \vx^{vir} = \vx + \lambda_1 \hat{\ve},
\end{gathered}
\end{equation}
where $\lambda_1$ is the coefficient that controls the degree of perturbation.

While the visual perturbation reveals the underlying virtual samples, we may unexpectedly incorporate some noisy samples resulting in the distribution shifts. We argue that the prototype of each class should be invariant when introducing virtual samples. Thus, in order to avoid distribution shift, we aim to fix the prototype for each class when perturbing the real samples. A class prototype is defined as the mean vector of the samples in the same class from the empirical distribution $p_{\bar{X}}$:
\begin{equation}
\begin{gathered}
  \mathbb{E}_{\vx_c \sim p_{\bar{X}}^{c}}[\bar{\vx}_c] = \frac{1}{N_c} \sum_{i=1}^{N_c}\vx_c^i,
\end{gathered}
\end{equation}
where $N_c$ is the sample number of the $c$-th class in the training set.

When generating a visual sample conditioned on $c$-th class with the corresponding semantic vector $\va_c$, the expected mean sample should be close to the class prototype given the prior $\vz$ as the mean vector from the prior distribution, \textit{i.e.,} all zeros $\bm{0}$:
\begin{equation}
\begin{gathered}
  \mathcal{L}_{proto} = \frac{1}{C_{s}} \sum^{C_{s}}_{c=1} \lVert f^{-1}(\bm{0},\va_{c}) - \mathbb{E}_{\vx_c \sim p_{\bar{X}}^{c}}[\bar{\vx}_c] \rVert^{2},
\label{proto}
\end{gathered}
\end{equation}
where $C_{s}$ is the number of seen classes. 

\subsection{Relative Positioning}
\label{gs}
To preserve the geometric information between different attribute categories in the shared subspace, we introduce the relative positioning technique.
% To enhance the inter-class relationship for unseen classes, we introduce the relative positioning technique, preserving the geometric information between different attribute categories in the shared subspace. 
Specifically, instead of representing the class-level semantic information using the raw attributes, we determine three semantic anchors to correspondingly obtain the relative position of each class in the attribute space. Such a relative position is defined as a global semantic vector, which could better aligns the semantic space with the visual one. 
%Specifically, instead of representing the class-level semantic information using the raw attributes, three semantic anchors are determined, based on which the relative position in the attribute space of each class in reference to the anchors is obtained. 

%The relative position of the raw attributes in the attribute space of each class is defined as a global semantic vector.
% By measuring the responses to a particular number of semantic anchors, we revise the semantic vectors to be global semantic representations.
% Due to the nature of the manual annotation, the collected attributes of class level semantic information are relatively sparse. Thus, the relationship between classes are implicit and not fully exploited. In this case, we aim to learn more representative semantic representations.

The process of determining the three semantic anchors is described as follows. We begin with constructing a semantic graph with the class-level semantic vectors. The edges $\mathcal{E}$ are defined as the cosine similarities between all semantic vectors:
\begin{equation}
\begin{gathered}
  \mathcal{E}_{ij} = \frac{\va_i\cdot\va_j}{\lVert\va_i \rVert_2 \cdot \lVert\va_j \rVert_2},
\end{gathered}
\end{equation}
where $\mathcal{E}_{ij}$ refers to the similarity between $i$-th class and $j$-th class. Then, for each class, we calculate the sum similarities to all other classes:
\begin{equation}
\begin{gathered}
  \vd_{i} = \sum_{j=1}^{C_s}\mathcal{E}_{ij},
\end{gathered}
\end{equation}
where $C_s$ denotes the total number of seen classes. We define the three semantic anchors $\va_{max}$,  $\va_{min}$, $\va_{med}$ with the highest, lowest, and median sum similarities to other semantic vectors. The global semantic vectors are then acquired by computing the responses from these three semantic anchors.

The dimensionality of visual features is usually much higher than that of semantic vectors, \textit{e.g.,} 2,048 vs. 85 in the AWA dataset. Thus, the generation process can be potentially dominated by visual features. In Section \ref{hpa}, we discuss the impact of the semantic vectors' dimensionality. To avoid this issue, we apply three functions $h_{max}(\cdot),h_{min}(\cdot),h_{med}(\cdot)$ to map the semantic responses to a higher dimension through the implementation with an FC layer and a ReLU activation function. The global semantic vector for each class can then be formulated as:
\begin{equation}
\begin{gathered}
  \va^{g}_{i} =  h_{max}(\va_{i} - \va_{max}) + h_{min}(\va_{i} - \va_{min}) + h_{med}(\va_{i} - \va_{med}).
%   \va^{g}_{i} = \sum_{\va_{*} \in \mathcal{A}^{g}} h(\va_{i} - \va_{*}),
\end{gathered}
\end{equation}
The global semantic vectors revised by relative positioning are fed into the conditional generation flow as the conditional information.
% where $\va_{*}$ represents one of the representative semantic representations in $\mathcal{A}^{g}$, and $\va_{i} - \va_{*}$ is the response from the specific representative semantic representation.


\subsection{Training and Zero-shot Inference}
% We have demonstrated our improving strategies for visual and semantic spaces, and also the conditional generative flow. In this subsection, we will illustrate the training strategy and zero-shot inference stage.

With the derived virtual samples $\vx^{vir}$ and the global semantic vectors $\va^{g}$, the objective functions $\mathcal{L}_{flow}$ and $\mathcal{L}_{proto}$ in Equation \ref{flow} and Equation \ref{proto} should be rewritten as:
\begin{equation}
\begin{gathered}
\mathcal{L}_{flow} = \mathbb{E}[-\log p_{X}(\vx^{vir};\va^{g},\theta)] - \log(p_{\theta}(\theta)), \\
\mathcal{L}_{proto} = \frac{1}{C_{s}} \sum^{C_{s}}_{c=1} \lVert f^{-1}(\bm{0},\va^{g}_{c}) - \mathbb{E}_{\vx_c \sim p_{\bar{X}}^{c}}[\bar{\vx}_c] \rVert^{2}.
 \end{gathered}
\end{equation}

Then, the overall objective function of the proposed GSMFlow is formulated as:
\begin{equation}
\begin{gathered}
  \underset{\theta}{min}( \mathcal{L}_{flow} + \lambda_2 \mathcal{L}_{proto}),
\end{gathered}
\end{equation}
where $\lambda_2$ is the coefficient of the prototype loss.

After the conditional generative flow is trained on the seen classes with the virtual samples and the global semantic vectors, it is leveraged to generate visual features of unseen classes:
\begin{equation}
\begin{gathered}
\bar{\vx}^{u} = g(\vz;\va^g, \theta).
\end{gathered}
\end{equation}
A softmax classifier is then trained on the real visual features of seen classes and the synthesized visual features of unseen classes. For the coming test samples from either seen or unseen classes, the softmax classifier aims to predict the corresponding class label accurately.

==> files/sections/experiments.tex <==
% \begin {table}
% \caption {Statistics of the four zero-shot learning datasets. }
% \begin{center}
% \scalebox{1.1}{
% \begin{tabular}{lccccc}
% \toprule
% \specialrule{.1em}{.00em}{.0em}
% \rowcolor[gray]{.9} Dataset             & aPaY          & AWA       & CUB   & FLO    \\
% % \specialrule{.1em}{.00em}{.00em}
% \specialrule{.1em}{-0.15em}{.1em}
% \# of Attributes     & 64           & 85        & 1024    & 1024   \\
% \# of Seen Classes   & 20           & 40        & 150    & 82     \\
% \# of Unseen Classes & 12           & 10        & 50     & 20     \\
% \# of Total Images   & 18,627       & 30,475    & 11,788 & 8,189  \\ \bottomrule \specialrule{.1em}{-.15em}{.00em}
% \end{tabular}}
% \end{center}
% \label{dataset}
% \vspace{-10pt}
% \end{table}  


\begin {table*}[t]
\caption {Performance comparison in accuracy (\%) of the state-of-the-art ZSL and GZSL on four datasets. For ZSL, performance results are reported with the average top-1 classification accuracy (T1). For GZSL, results are reported in terms of top-1 accuracy of unseen (U) and seen (S) classes, together with their harmonic mean (H). The best results of the harmonic mean are highlighted in bold. $\dag$ and $\ddag$ represent embedding-based and generative methods, respectively.}
% \begin{center}
\centering
\scalebox{0.95}{
\begin{tabular}[t]{c|c|cccc|cccc|cccc|cccc}
\specialrule{.1em}{.00em}{.00em}
 \rowcolor[gray]{.9} \multirow{2}{*}{} &  \multirow{2}{*}{}   & \multicolumn{4}{c|}{aPaY}   & \multicolumn{4}{c|}{AWA}  &  \multicolumn{4}{c|}{CUB} & \multicolumn{4}{c}{FLO}  \\  \hhline{>{\arrayrulecolor [gray]{0.9}}-->{\arrayrulecolor {black}}----------------} % \cmidrule[.1em]{3-18}


\rowcolor[gray]{.9}  & \multirow{-2}{*}{Methods}  & \multicolumn{1}{c|}{\textit{T1}} &\textit{U} & \textit{S} & \textit{H}  & \multicolumn{1}{c|}{\textit{T1}} & \textit{U} & \textit{S} & \textit{H}  & \multicolumn{1}{c|}{\textit{T1}} & \textit{U} & \textit{S} & \textit{H} & \multicolumn{1}{c|}{\textit{T1}} & \textit{U} & \textit{S} & \textit{H}\\

  \specialrule{.1em}{.00em}{.00em}
\multirow{6}{*}{\dag}   
                      &   LATEM   \cite{xian2016latent}  
&\multicolumn{1}{c|}{35.2}    & 0.1           & 73.0              & 0.2        
&\multicolumn{1}{c|}{55.8}    & 13.3          & 77.3              & 20.0
&\multicolumn{1}{c|}{49.3}    & 15.2          & 57.3              & 24.0    
&\multicolumn{1}{c|}{60.8}    & 6.6           & 47.6              & 11.5  
    \\
 
                      &   ALE    \cite{akata2015label}   
&\multicolumn{1}{c|}{39.7}    & 4.6           & 73.7              & 8.7      
&\multicolumn{1}{c|}{62.5}    & 14.0          & 81.8              & 23.9    
&\multicolumn{1}{c|}{54.9}    & 23.7          & 62.8              & 34.4    
&\multicolumn{1}{c|}{48.5}    & 13.3          & 61.6              & 21.9  
    
    \\
                   &   SJE       \cite{akata2015evaluation}
&\multicolumn{1}{c|}{31.7}    & 1.3          & 71.4              & 2.6       
&\multicolumn{1}{c|}{61.9}    & 8.0          & 73.9              & 14.4  
&\multicolumn{1}{c|}{54.0}    & 23.5         & 59.2              & 33.6      
&\multicolumn{1}{c|}{53.4}    & 13.9         & 47.6              & 21.5    
    \\
    %                 &      ESZSL       \cite{romera2015embarrassingly}
    % & 2.4          & 70.1              & 4.6       
    % & 5.9          & 77.8              & 11.0  
    % & 14.7         & 56.5              & 23.3      
    % & -            & -                 & -    
    % \\

                    & SAE     \cite{kodirov2017semantic}  
&\multicolumn{1}{c|}{8.3}    & 0.4           & 80.9              & 0.9        
&\multicolumn{1}{c|}{54.1}    & 1.1           & 82.2              & 2.2 
&\multicolumn{1}{c|}{33.3}    & 7.8           & 54.0              & 13.6
&\multicolumn{1}{c|}{-}    & -             & -                 & -    
    \\

                    & TCN       \cite{jiang2019transferable}
&\multicolumn{1}{c|}{38.9}    & 24.1          & 64.0              & 35.1       
&\multicolumn{1}{c|}{71.2}    & 61.2          & 65.8              & 63.4
&\multicolumn{1}{c|}{59.5}    & 52.6          & 52.0              & 52.3      
&\multicolumn{1}{c|}{-}    & -             & -                 & -    
    \\
                    & DVBE      \cite{min2020domain}
&\multicolumn{1}{c|}{-}    & 32.6          & 58.3              & 41.8          
&\multicolumn{1}{c|}{-}    & 63.6          & 70.8              & 67.0     
&\multicolumn{1}{c|}{-}    & 53.2          & 60.2              & 56.5         
&\multicolumn{1}{c|}{-}    & -             & -                 & -   
    \\

 \specialrule{.1em}{.20em}{.20em}
\multirow{10}{*}{\ddag} & GAZSL \cite{zhu2018generative}      
&\multicolumn{1}{c|}{41.1}    & 14.2          & 78.6              & 24.0      
&\multicolumn{1}{c|}{70.2}    & 35.4	        & 86.9              & 50.3   
&\multicolumn{1}{c|}{55.8}    & 31.7	        & 61.3	            & 41.8       
&\multicolumn{1}{c|}{60.5}    & 28.1          & 77.4              & 41.2 
    \\

                        & f-CLSWGAN \cite{xian2018feature}     
&\multicolumn{1}{c|}{40.5}   & 32.9           & 61.7              & 42.9    
&\multicolumn{1}{c|}{65.3}   & 56.1           & 65.5              & 60.4     
&\multicolumn{1}{c|}{57.3}   & 43.7           & 57.7              & 49.7	       
&\multicolumn{1}{c|}{69.6}   & 59.0           & 73.8              & 65.6 
   \\
                     &  CANZSL   \cite{chen2020canzsl}         
&\multicolumn{1}{c|}{-}    & -                 & -                 & -  
&\multicolumn{1}{c|}{68.9}    & 49.7              & 70.2              & 58.2  
&\multicolumn{1}{c|}{60.6}    & 47.9              & 58.1              & 52.5 
&\multicolumn{1}{c|}{69.7}    & 58.2              & 77.6              & 66.5 
    \\
    %                 &  cycle-CLSWGAN   \cite{felix2018multi}         
    % & -                 & -                 & -  
    % & 56.9              & 64.0              & 60.2  
    % & 45.7              & 61.0              & 52.3 
    % & 59.2              & 72.5              & 65.1 
    % \\
 
                    & CADA-VAE  \cite{schonfeld2019generalized}
&\multicolumn{1}{c|}{42.3}    & 31.7              & 55.1              & 40.3     
&\multicolumn{1}{c|}{64.0}    & 55.8              & 75.0              & 63.9     
&\multicolumn{1}{c|}{60.4}    & 51.6              & 53.5              & 52.4     
&\multicolumn{1}{c|}{65.2}    & 51.6              & 75.6              & 61.3 
    \\        
                    & f-VAEGAN-D2  \cite{xian2019f} 
&\multicolumn{1}{c|}{-}    & -                 & -                 & -         
&\multicolumn{1}{c|}{71.1}    & 57.6              & 70.6              & 63.5     
&\multicolumn{1}{c|}{61.0}    & 48.4              & 60.1              & 53.6     
&\multicolumn{1}{c|}{67.7}    & 56.8              & 74.9              & 64.6 
    \\       
                 
             
                    & TF-VAEGAN  \cite{narayan2020latent}
&\multicolumn{1}{c|}{-}    & -                 & -                 & -     
&\multicolumn{1}{c|}{72.2}    & 59.8              & 75.1              &  66.6  
&\multicolumn{1}{c|}{64.9}    & 52.8              & 64.7              & 58.1       
&\multicolumn{1}{c|}{70.8}    & 62.5              & 84.1              & 71.7  
    \\

                    & E-PGN  \cite{yu2020episode}
&\multicolumn{1}{c|}{-}    & -                 & -                 & -          
&\multicolumn{1}{c|}{73.4}    & 52.6              & 83.5              & 64.6    
&\multicolumn{1}{c|}{72.4}    & 52.0              & 61.1              & 56.2 
&\multicolumn{1}{c|}{85.7}    & 71.5              & 82.2              & 76.5  
     
    \\ 
        & IZF \cite{shen2020invertible}
&\multicolumn{1}{c|}{44.9}    & 42.3              & 60.5              & 49.8
&\multicolumn{1}{c|}{\textbf{74.5}}    & 60.6              & 77.5              & 68.0    
&\multicolumn{1}{c|}{67.1}    & 52.7              & 68.0              & 59.4    
&\multicolumn{1}{c|}{-}    & -                 & -                 & -  
     
    \\ 
          & OOD-GZSL \cite{chen2020boundary}
&\multicolumn{1}{c|}{-}    & -                 & -                 & -          
&\multicolumn{1}{c|}{-}    & 55.9              & 94.9              & 70.3    
&\multicolumn{1}{c|}{-}    & 53.8              & 94.6             &\textbf{68.6}
&\multicolumn{1}{c|}{-}    & 61.9              & 91.7              & 73.9  
     
    \\  
          & SDGZSL \cite{chen2021iccv}
&\multicolumn{1}{c|}{45.4}    & 38.0              & 57.4              & 45.7          
&\multicolumn{1}{c|}{72.1}    & 64.6              & 73.6              & 68.8    
&\multicolumn{1}{c|}{75.5}    & 59.9              & 66.4         &63.0
&\multicolumn{1}{c|}{\textbf{86.9}}    & 83.3              & 90.2             & 86.6  
     
    \\  
    
\specialrule{.1em}{.00em}{.00em}

\rowcolor[gray]{.9} &   GSMFlow
&\multicolumn{1}{c|}{\textbf{49.2}} & 42.0 & 62.3 & \textbf{50.2}  
&\multicolumn{1}{c|}{72.7} & 64.5 & 82.1 & \textbf{72.3}
&\multicolumn{1}{c|}{\textbf{76.4}} & 61.4 & 67.4 & 64.3
&\multicolumn{1}{c|}{\textbf{86.9}} & 86.6 & 87.8 & \textbf{87.2} 
\\
\specialrule{.1em}{.00em}{.00em}
\end{tabular}}
\label{gzslperoformance}
\end {table*} 

In this section, we evaluate our approach GSMFlow in both generalized zero-shot learning and conventional zero-shot learning tasks. We first introduce the datasets and experimental settings and then compare GSMFlow with the state-of-the-art methods. Finally, we study the effectiveness of the proposed model with a series of ablation study and hyper-parameter sensitivity analysis. 

\subsection{Datasets}
We conduct experiments on four widely used benchmark datasets of image classification. They are two fine-grained datasets, \textit{i.e.,} Caltech-UCSD Birds-200-2011 (\textbf{CUB}) \cite{wah2011caltech} and Oxford  Flowers (\textbf{FLO}) \cite{nilsback2008automated}, two coarse-grained datasets, \textit{i.e.,} Attribute Pascal and Yahoo (\textbf{aPaY}) \cite{farhadi2009describing} and Animals with Attributes 2 (\textbf{AWA}) \cite{lampert2013attribute}.
CUB consists of 11,788 images from 200 fine-grained bird species, in which 150 selected as seen classes and 50 as unseen classes. For FLO, it contains 8,189 images from 102 flower categories, 82 of which are chosen as seen classes. The class-level semantic vectors of CUB and FLO are extracted from the fine-grained visual descriptions (10 sentences per image), yielding 1,024-dimensional character-based CNN-RNN features \cite{reed2016learning} for each class. aPaY dataset contains 18,627 images from 42 classes. There are 30 seen classes and 12 unseen classes respectively. Each class is annotated with 64 attributes. AWA2 is a considerably larger dataset with 30,475 images from 50 classes and they are annotated with 85 attributes. For the split, 40 of the total classes are selected as seen classes and ten as unseen classes. For each dataset, We follow the proposed split setting in \cite{xian2018zero} and \cite{nilsback2008automated}. 
% The specific statistics is illustrated in Table  \ref{dataset}.


\subsection{Implementation Details}
Our framework is implemented with the open-source machine learning library PyTorch. The conditional generative flow consists of a series of affine coupling layers. Each affine coupling layer is implemented with two fully connected (FC) layers and the first FC layer is followed by a LeakyReLU activation function. The hidden dimension of the FC layer is set as 2,048. The coefficients $\lambda_1$ of perturbation degree and the coefficient $\lambda_2$ of the prototype loss are set within \{0.02, 0.05, 0.15, 0.3, 0.5\} and \{1, 3, 10, 20, 30\}. The dimension of global semantic vectors varies in \{128, 256, 512, 1,024, 2,048\} and the number of the affine coupling layers varies in \{1, 3, 5, 10, 20\}.  The corresponding results are given in Section \ref{hpa}. The function $h(\cdot)$ is implemented with an FC layer and a ReLU activation function. We use Adam optimizer with $\beta_{1}=0.9$, $\beta_{2}=0.999$ and set the batch size to 256 and set the learning rate to 3e-4. All the experiments are performed on a Lenovo workstation with two NVIDIA GeForce GTX 2080 Ti GPUs.


\subsection{Evaluation Metrics}
To avoid the failure of classification accuracy for imbalanced class distributions, we adopt average per-class Top-1 accuracy as the fair evaluation criteria for conventional ZSL and the seen and unseen set performance in GZSL:
\begin{equation}
\begin{aligned}
  Acc_{\mathcal{Y}} = \frac{1}{|\mathcal{Y}|} \sum^{|\mathcal{Y}|}_{y=1} \frac{\# \  of \ correct \ predictions \ in \ y}{\# \ of \ samples \ in \ y},
\end{aligned}
\end{equation}
where $|\mathcal{Y}|$ is the number of testing classes. A correct prediction is defined as the highest probability of all candidate classes.
Following \cite{xian2018zero}, the harmonic mean of the average per-class Top-1 accuracies on seen $Acc_S$ and unseen $Acc_U$ classes are used to evaluate the performance of generalized zero-shot learning. It is computed by:
\begin{equation}
\begin{aligned}
  H = \frac{2*Acc_S*Acc_U}{Acc_S+Acc_U}.
\end{aligned}
\end{equation}



\subsection{Comparisons with State-of-the-art Methods}
\label{GZSL}

Table \ref{gzslperoformance} summarizes the performance comparison between our proposed GSMFlow and the other state-of-the-art methods in the setting of GZSL. We choose the most representative state-of-the-art methods for comparison, the top six methods marked with $\dag$ are embedding-based methods, while the below eleven methods and our proposed method marked with $\ddag$ are generative methods. The unseen, seen and the balanced harmonic mean between the two domains are represented as U, S, and H. It can be seen that our proposed framework consistently outperforms other methods except on CUB dataset. It is worth noting that  OOD-ZSL achieves the best performance on CUB as it leverages a specific calibration technique to threshold the confidence of the prediction being seen or unseen. The thresholding hyperparameter is sensitive to the datasets, which makes it hard to generalize when more unseen classes are involved. Among the generative methods, IZF \cite{shen2020invertible} also leverages normalizing flows as the base generative model.
However, we show that by mitigating the generation shifts, our proposed GSMFlow achieves significant improvements on these four datasets. 


% As the groundtruth visual features of unseen classes are unavailable during training, we cannot capture the real distribution of unseen classes. Thus, the negative MMD loss in IZF is an unstable component to push the distribution of synthesized unseen visual features away from the distribution of visual features of seen classes. By increasing the divergence between seen and unseen classes, it may cause unexpected distribution shifts between the synthesized visual features and the real unseen visual features. As the source code of this paper is not publicly available, we try to reproduce the negative MMD loss. However, it degrades the performance, and we observe that the detrimental effect discussed above. We also improve the approach that how they handle conditional information in the generative model. By repeatedly injecting the semantic information into each of the coupling layers, the synthesized visual features are more semantic consistent.


% \begin {table}[t]
% \caption {Conventional ZSL accuracy (\%). The best results are formatted in bold.}
% \begin{center}
% \scalebox{1.}{
% \begin{tabular}[h]{ l | c | c | c | c  }
% \specialrule{.1em}{.00em}{.00em}
%   \rowcolor[gray]{.9}  Method & aPaY & AWA & CUB & FLO \\
%   \specialrule{.1em}{.00em}{.00em}

%   ALE   \cite{akata2015label}             
%                     & 39.7      & 62.5      & 54.9          & 48.5          \\
%   SJE   \cite{akata2015evaluation}          
%                     & 31.7      & 61.9      & 54.0          & 53.4          \\
%   ESZSL \cite{romera2015embarrassingly}           
%                     & 38.3      & 58.6      & 51.9          & 51.0          \\
%   LFGAA \cite{liu2019attribute}   
%                     & -         & 68.1      & 67.6          & -          \\
%   DCN \cite{liu2018generalized}
%                     & 43.6      & 65.2      & 56.2          & -          \\
%   TCN \cite{jiang2019transferable}
%                     & 43.6      & 65.2      & 56.2          & -          \\
%   GAZSL \cite{zhu2018generative}      
%                     & 41.1      & 70.2      & 55.8          & 60.5	        \\
%   f-CLSWGAN \cite{xian2018feature}     
%                     & 40.5      & 65.3      & 57.3          & 69.6          \\
%   cycle-CLSWGAN  \cite{felix2018multi}         
%                     & -         & 66.8      & 58.6          & 70.3          \\
%   CADA-VAE  \cite{schonfeld2019generalized}
%                     & -         & 64.0      & 60.4          & -             \\        
%   f-VAEGAN-D2  \cite{xian2019f} 
%                     & -         & 71.1      & 61.0          & 67.7          \\       
%   DLFZRL  \cite{tong2019hierarchical}
%                     & 46.7      & 70.3      & 61.8          & -             \\       
%   TF-VAEGAN  \cite{narayan2020latent}
%                     & -         & 72.2      & 64.9          & 70.8           \\
%   E-PGN  \cite{yu2020episode}
%                     & -         & 73.4      & 72.4          & 85.7           \\
%   IZF  \cite{shen2020invertible}
%                     & 44.9         & \textbf{74.5}      & 67.1          & -           \\
% \specialrule{.1em}{.00em}{.00em}
%  \rowcolor[gray]{.9} GSMFlow          & \textbf{49.2}    & 72.7      & \textbf{76.4}          & \textbf{86.9}  \\
% \specialrule{.1em}{.00em}{.20em}
% \end{tabular}}
% \end{center}
% \label{czsl}
% \end {table}


\subsection{Conventional Zero-shot Learning}
\label{ZSL}
Even if GSMFlow is mainly proposed for GZSL, to further validate the effectiveness of our proposed framework, we also conduct experiments in the context of conventional ZSL. Table \ref{gzslperoformance} summarizes the conventional zero-shot learning performance, which is reported under the T1 metric. We achieve better performance than all the compared methods on the aPaY, CUB, and FLO datasets. For the AWA dataset, we can also achieve comparatively good performance. 

\begin {table}[t]
\caption {Effects of different components on aPaY and AWA datasets. U, S and H represent unseen, seen and harmonic mean, respectively. The best results of harmonic mean are formatted in bold.}
\begin{center}
\scalebox{0.91}{
\begin{tabular}[t]{c|ccc|ccc}
\specialrule{.1em}{.00em}{.00em}
  \rowcolor[gray]{.9}     & \multicolumn{3}{c|}{aPaY} & \multicolumn{3}{c}{AWA}   \\  \rowcolor[gray]{.9} Settings
   & \textit{U} & \textit{S} & \textit{H}  & \textit{U} & \textit{S} & \textit{H}  \\

    \specialrule{.1em}{-.15em}{.00em}
  IZF w/o constraints      & 35.2      & 54.2     & 42.7      
            & 38.1      & 78.9      & 51.4   
            \\

  GSMFlow w/o constraints   
            & 36.5      & 60.0      & 45.4       
            & 53.3      & 67.6      & 59.6   
            \\

  GSMFlow w/o VP     
            & 38.4      & 62.3      & 47.6        
            & 62.2      & 71.3      & 66.4   
            \\

 GSMFlow w/o RP
            & 39.6      & 61.3      & 48.1         
            & 62.9      & 80.4      & 70.6
            \\

    \specialrule{.1em}{.10em}{.00em}

 \rowcolor[gray]{.9} GSMFlow      
& 42.0 & 62.3 & \textbf{50.2}  
& 64.5 & 82.1 & \textbf{72.3}
\\

\specialrule{.1em}{.00em}{.00em}
\end{tabular}}
\end{center}
\label{ablation}
\end {table}


\subsection{Ablation Study}
% \subsection{Model Analysis}
% \noindent \textbf{Ablation Study}
To analyze the contribution of each proposed component and the merit from addressing the three problems in generative zero-shot learning, \textit{i.e., semantic inconsistency, variance dacay}, and \textit{structure disorder}, we conduct an ablation study on the proposed GSMFlow. We decompose the complete framework into four variants. These include: \textit{\textbf{IZF w/o constraints}} - the conditional generative flow adopted in compared method \cite{shen2020invertible}; \textit{\textbf{GSMFlow w/o constraints}} - the generative flow in our proposed framework without visual perturbation and global semantic learning; \textit{\textbf{GSMFlow w/o VP}} - the complete framework without visual perturbation; and \textit{\textbf{GSMFlow w/o RP}} - the original class-level semantic vectors are used. 

Comparing between \textit{\textbf{IZF w/o constraints}} and \textit{\textbf{GSMFlow w/o constraints}}, we can see the performance comparison between the two ways of incorporating conditional information in the generative flow. It can be seen that, instead of mixing the conditional information with the prior input in IZF, our explicit conditional strategy that progressively injects the semantic information into the affine coupling layers during training can achieve higher accuracy on GZSL. 
The results on the variants \textit{\textbf{GSMFlow w/o VP}} shows that by mitigating the structure disorder issue, the relative positioning strategy that captures geometric relationships between semantic vectors can significantly improve the GZSL performance. 
\textit{\textbf{GSMFlow w/o RP}} indicates that effectiveness of the visual perturbation strategy to prevent the variance collapse. When combining these components together, we achieve the best performance results.
\begin{figure}[t]
\centering
\includegraphics[width=85mm]{files/graphics/cm.pdf}
\caption{Class-wise performance comparison between with and without visual perturbations. The vertical labels are the groundtruth and the horizontal labels are the predictions.}
\label{cm}
\end{figure}


\begin{figure*}[t]
\centering
\includegraphics[width=175mm]{files/graphics/tsne.pdf}
\caption{Distribution comparison of the unseen classes in the AWA dataset. (a) The real distributions of the visual features extracted from the backbone. (b) The synthesized distributions by cGAN. (c) The synthesized distributions by GSMFlow.}
\label{tsne}
\end{figure*}

\begin{figure}[t]
\centering
\includegraphics[width=85mm]{files/graphics/hyper.pdf}
\caption{Hyper-parameter sensitivity. The horizontal axis indicates the varying hyper-parameters for (a) perturbation weight, (b) prototype loss weight, (c) semantic vector dimensions, and (d) number of affine coupling layers. The vertical axis reports the corresponding performance.}
\label{hyper}
\end{figure}

\subsection{Class-wise Performance Comparison}
To further investigate the performance boost through visual perturbation, in Figure \ref{cm}, we compare the class-wise accuracy with and without visual perturbation by illustrating the confusion matrices in the two settings on AWA dataset. Without visual perturbation. We argue that by perturbing the visual features, the generator is exposed to more diverse visual samples, resulting in better generalization ability to unseen classes. Especially, in this case study, the \textit{horses} and the \textit{sheep} are the two unseen classes in AWA dataset. We can notice that \textit{horses} can be easily misclassified as \textit{sheep} and can only achieve 14\% accuracy. The performance surges to 55\% when we introduce the visual perturbation strategy. Similar observations hold for other classes.

\subsection{Hyper-parameter Analysis}
\label{hpa}
GSMFlow mainly involves four hyper-parameters in the model training, as shown in Figure \ref{hyper}. Varying the perturbation weight $\lambda_1$ from 0.02 to 0.5, in Figure \ref{hyper}(a), we find that the aPaY and AWA can reach the peak at around 0.02 and 0.15, respectively. 
It turns out that the weight of the prototype loss $\lambda_2$ does not have a significant impact on the performance.
In Figure \ref{hyper}(b), we vary $\lambda_2$ between 1 and 30, and observe that at 3 and 10, the best performance results are achieved on aPaY and AWA2. 
As discussed in Section \ref{gs}, the semantic vectors usually have lower dimensions than the visual features, which makes the visual features dominate the generation process in the affine coupling layers. 
In Figure \ref{hyper}(c), we report the impact from the dimensionality of the semantic vectors. It can be seen that low-dimensional semantic vectors tend to jeopardize the performance. The best performance results are both achieved at 1,024 dimensions. 
We also investigate the impact on the number of conditional affine coupling layers, which directly influences the generative model size. In Figure \ref{hyper}(d), we can see the best performance results are from 3 and 5 layers respectively for the aPaY and AWA datasets. 


\subsection{t-SNE visualization}
The quantitative results reported for GZSL (Section \ref{GZSL}) and ZSL (Section \ref{ZSL}) demonstrate that the visual samples of the unseen classes generated by GSMFlow are of good quality and effective for classification tasks. 
To further gain an insight into the quality of the generated samples and validate the motivation illustrated in Figure \ref{intro}, we compare the empirical distribution of the real unseen class data and the synthesized unseen class data by a conditional generative adversarial network (cGAN) and our proposed GSMFlow, as depicted in Figure \ref{tsne}. 
It can be seen that the distributions of the synthesized unseen data from cGAN suffer from the generation shifts problem, which is undesirable for approximating optimal decision boundaries. Specifically, each class is collapsed to fixed modes without capturing enough variances. 
In contrast, thanks to the visual perturbation strategy, the synthesized samples by GSMFlow are much more diverse, which helps to approximate optimal decision boundaries. The class-wise relationship is also reflected. 
For example, comparing to other animal species, \textit{horse} and \textit{giraffe} share some attribute values. Also, all the marine species, \textit{blue whale, walrus, dolphin, and seal} are well separated from other animals. 
As a result, the generated samples are semantically consistent.


==> files/sections/introduction.tex <==
Deep learning techniques have significantly boosted the performance of many tasks in computer vision \cite{wang2020prototype,luo2020learning}. However, the performance gains come at the cost of an enormous amount of labeled data. Generally, shallow classification algorithms need a certain amount of training data of every class, while deep learning dramatically amplifies the need. Data labeling is time-consuming and expensive, even if the raw data is usually plentiful. Moreover, it is unrealistic to require labeled data for every class, leading extra attention from researchers drawn to Zero-Shot Learning (ZSL) as a solution \cite{akata2015label,xian2016latent,akata2015evaluation,yang2016zero,li2019zero}. By incorporating side information, \textit{e.g.,} class-level semantic attributes, ZSL transfers semantic-visual relationships from the seen classes to unseen classes without any visual samples. While conventional ZSL aims to recognize only unseen classes, it is infeasible to assume that we will only come across samples from unseen classes. Hence, in this paper, we consider a more realistic and challenging task, Generalized Zero-Shot Learning (GZSL), to classify over both seen and unseen classes \cite{huang2019generative,schonfeld2019generalized,xian2018feature,li2020learning}.

\begin{figure}[t]
\centering
\includegraphics[width=85mm]{files/graphics/intro.pdf}
\caption{ An illustration of the generation shifts. 
% An illustration of the distribution collapse problem. 
a) Implicit semantic encoding causes the semantic inconsistency when generating unseen samples. b) The synthesized samples collapse to fixed modes. c) The synthesized samples fail to fully preserve the geometric relationships in the semantic space.
% (a) The real distribution of the unseen classes. (b) As the variance of the unseen classes cannot be captured, the synthesized distribution collapses to fixed modes.
}
\label{intro}
\vspace{-12pt}
\end{figure}

GZSL can be roughly categorized into embedding-based methods \cite{xian2016latent,akata2015label,akata2015evaluation,xie2020region} and generative methods \cite{li2019leveraging,xian2018feature,schonfeld2019generalized,li2019alleviating,xie2021generalized}. 
Embedding-based methods usually cast the semantic and visual features into the same space, where the compatibility scores between the visual features and all classes are computed for predictions. In contrast, generative methods \cite{long2017zero,xian2018feature,schonfeld2019generalized,chen2020rethinking,shen2020invertible,li2021investigating} cast the GZSL problem into a supervised classification task by generating synthesized visual features for unseen classes. 
Then a supervised classifier can be trained on both real seen visual features and the synthesized unseen visual features. 
% Our approach takes GZSL from the generative perspective.

\begin{figure*}[t]
\centering
\includegraphics[width=175mm]{files/graphics/architecture.pdf}
\caption{An illustration of the proposed GSMFlow framework. The conditional generative flow is comprised of a series of conditional affine coupling layers. Particularly, the perturbation is injected into the original visual features to complement the potential patterns and the global semantics are computed with relative positioning to semantic anchors. For inference, a latent variable $\vz$ is inferred from the visual features of an image sample $\vx$ conditioned on a global semantic vector $\va^g$. Inversely, given $\vz$ drawn from a prior distribution and a global semantic vector $\va^g$, GSMFlow can generate a visual sample accordingly.}
% Through the conditional affine coupling layers conditioned on a semantic vector $\va$.}
\label{architecture}
\vspace{-8pt}
\end{figure*}

% Unseen Visual Data Synthesis (UVDS) \cite{long2017zero} is the pioneering work that initiates the generative paradigm in zero-shot learning. In the following works, Generative Adversarial Nets (GANs) \cite{goodfellow2014generative}, Variational Autoencoders (VAEs) \cite{VAE}, and some hybrid models, \textit{e.g.,} VAE-GAN \cite{bao2017cvae}, are widely adopted. f-CLSWGAN \cite{xian2018feature} presents a conditional WGAN-based \cite{arjovsky2017wasserstein} generative model to synthesize plausible visual features. 
% CADA-VAE \cite{schonfeld2019generalized} proposes a stacked VAE architecture that is comprised of two VAEs for the semantic and visual spaces, respectively. The latent spaces of the two VAEs are aligned to shared the invariant information between semantic and visual spaces.
% SE-ZSL \cite{verma2018generalized} proposes a conditional VAE model coupled with a regressor network to provide feedback to the generator. 
% MPGAN \cite{chen2020rethinking} considers generative ZSL from the ensemble perspective, which synthesizes the visual patches independently and predicts class labels based on different patches' attention weights. 

In spite of the advances achieved by the generative paradigm, the synthesized visual features may not be guaranteed to cover the real distribution of unseen classes, given that the unseen features are not exposed during training.
Due to the gap between the synthesized and the real distributions of unseen features, the trained classifier tends to misclassify the unseen samples.
Therefore, it is critical to analyze the causes and mitigate the resulted generation shifts. In this paper, as illustrated in Figure \ref{intro}, we identify three common types of generation shifts in generative zero-shot learning methods:
\begin{itemize}
    \item \textbf{Semantic inconsistency:} The state-of-the-art GZSL approach \cite{shen2020invertible} focuses on preserving the exact generation cycle consistency by a normalizing flow. It constructs a complex prior and disentangle the outputs into semantic and non-semantic vectors. Such implicit encoding may cause the generated samples to be incoherent with the given attributes and deviated from the real distributions.
    \item \textbf{Variance collapse:} The synthesized samples commonly collapse into fixed modes and fail to capture the intra-class variance of unseen samples, which can be originated from different poses, illumination and background.
     \item \textbf{Structure disorder:} It is also hard to fully preserve the geometric relationships between different attribute categories in the shared subspace. If the relative position of unseen samples changes in the visual space, the recognition performance will inevitably degenerate. 
\end{itemize}

% In spite of the advances achieved by the generative paradigm, the synthesized samples may not be guaranteed to cover the real distribution of unseen data points, since the unseen features are not exposed during training. When there is a gap between the synthesized and real unseen features, the trained classifier is prone to mis-classify unseen samples. Therefore it is critical to identify and mitigate the generation discrepancy. In this paper, we identify three common types of data shifts in generative models: (1) \textit{semantic inconsistency} (2) \textit{variance decay} and (3) \textit{structural shifts} as illustrated in Figure \ref{intro}. First, the state-of-the-art GZSL approaches \cite{chen2020canzsl,shen2020invertible} focus on preserving exact cycle consistency and constructing complex a prior and disentangle the outputs into semantic and non-semantic vectors. Such implicit encoding may cause the generated samples to be incoherent with the given attributes and deviated from the clusters. Second, the synthesized samples commonly collapse into fixeds modes and fail to capture the intra-class variance of unseen samples, which can be originated from different poses, illumination and background. Third, it is also hard to fully preserve the geometric relationship between different attributes categories in the shared subspace. If the relative position of unseen samples changes in the visual space, the recognition performance will inevitably degenerate.  

% In zero-shot learning, domain shift \cite{fu2015transductive} is a fundamental problem. It refers to the observation that although some classes share the same attributes, their visual appearances are reflected differently, \textit{e.g.,} the \textit{`hasTail'} attribute reflects different tail styles for \textit{`pig'} and \textit{`horse'}. 
% We argue that as the training stage only involves the seen data, the learned generative model may overfit the visual appearances of the seen data. According to the domain shift problem, in contrast, the visual appearances in the unseen classes are different. Hence, when generalizing to unseen classes, the generative model cannot reflect the visual variance of unseen classes, resulting in the collapsed distributions. 


% (1) 为了解决XXX, 我们显示地把Attribute 融合到forward 和backward 让生成的sample更 XXX
% (2) 为了Recover 真实的variance,我们在原始X空间插入noise，让infer出来的unseen更逼近
% （3）为了保留语义空间 类间结构关系，我们选择不同的anchor来correct attribute的representation


To address these potential generation shifts, in this paper, we propose a novel framework for generalized zero-shot learning, namely Generation Shifts Mitigating Flow (GSMFlow), as depicted in Figure \ref{architecture}. In particular, to tackle the semantic inconsistency, we explicitly embed the semantic information into the transformations in each of the coupling layers during inference and generation, enforcing the unseen visual feature generation to be semantically consistent. Furthermore, to mitigate the variance collapse issue, a visual perturbation strategy is proposed to diversify training samples by dynamically injecting the perturbation noise into the input samples. With this strategy, the decision boundary could be adjusted for suiting the real unseen samples at the test time. Moreover, to alleviate the semantic structure disorder, the relative positioning mechanism is adopted to correct the attribute representations by preserving the global geometrical relationship to the specific semantic anchors. 
Specifically, the visual features $\vx$ of a real sample are first extracted from a backbone network, \textit{e.g.,} ResNet101. In the inference stage, a real sample is perturbed to be a virtual sample, which is further fed into a conditional generative flow $f(\cdot)$. The inference process is conditioned on the manipulated global semantic vector to infer the latent factors drawn from a prior distribution. The learned generative flow has its inverse transformation as the generative network. Similarly, a global semantic vector is progressively injected into each of the inverse coupling layers to generate unseen visual features from latent factors. Eventually, a unified classifier is trained with the real seen features and the generated unseen features, aiming to accurately recognize both seen and unseen classes at the test time. To sum up, the contributions of our work are listed as follows\footnote{Our code is available at: {\href{https://github.com/uqzhichen/GSMFlow}{https://github.com/uqzhichen/GSMFlow}}.}:
\begin{itemize}
    \item 
    Aa novel GSMFlow framework is proposed for GZSL, which explicitly incorporates the class-level semantic information into both the forward and the inverse transformations of the conditional generative flow. It encourages the synthesized samples to be more coherent with the respective semantic information.  
    
    \item We propose a visual perturbation strategy to 
    imitate the intrinsic variance of unseen classes in synthesized samples. By injecting perturbation noise into the seen training sample, we diversify the training samples to enrich the original feature space. As the generative flow is exposed to more diverse virtual samples, the synthesized samples of unseen classes can thus capture more visual potentials.
   
    \item To preserve the geometric relationship between different semantic vectors in the semantic space, we choose different semantic anchors to revise the representation of the attributes.
    \item Comprehensive experiments and in-depth analysis on four GZSL benchmark datasets demonstrate the state-of-the-art performance by the proposed GSMFlow framework in the GZSL tasks.
\end{itemize}

The rest of the paper is organised as follows. We briefly review related work in Section 2. GSMFlow is presented in Section 3, followed
by the experiments and the in-depth analysis in Section 4. Lastly, Section 5 concludes the
paper.



==> files/sections/related_work.tex <==
\subsection{Traditional Zero-shot Learning}
Traditional solutions towards zero-shot learning are mostly the embedding-based methods. The pioneering method ALE \cite{akata2015label} proposes to employ embedding functions to measure the compatibility scores between a semantic embedding and a data sample. SJE \cite{akata2015evaluation} extends ALE by using structured SVM \cite{tsochantaridis2005large} and takes advantage of the structured outputs. DeViSE \cite{frome2013devise} constructs a deep visual semantic embedding model to map 4096-dimensional visual features from AlexNet \cite{krizhevsky2012imagenet} to 500 or 1000-dimensional skip-gram semantic embeddings. EZSL \cite{romera2015embarrassingly} theoretically gives the risk bound of the generalization error and connects zero-shot learning with the domain adaptation problem. More recently, SAE \cite{kodirov2017semantic} develops a cycle embedding approach with an autoencoder to reconstruct the learned semantic embeddings into a visual space. Later, the cycle architecture is also investigated in generative methods \cite{chen2020canzsl}. However, these early methods have not achieved satisfactory results on zero-shot learning. Particularly, when applying on the GZSL task, the unseen class performance is even worse. Recently, thanks to the advances of generative models, by generating missing visual samples of unseen classes, zero-shot learning can be converted into a supervised classification task.

\subsection{Generative GZSL}
A number of generative methods have been applied for GZSL, \textit{e.g.,} Generative Adversarial Nets (GANs) \cite{goodfellow2014generative}, Variational Autoencoders (VAEs) \cite{kingma2013auto}, and Alternating Back-Propagation algorithms (ABPs) \cite{han2017alternating}. f-CLSWGAN \cite{xian2018feature} presents a WGAN-based \cite{arjovsky2017wasserstein} approach to synthesize unseen visual features based on semantic information. CADA-VAE \cite{schonfeld2019generalized} proposes to stack two VAEs, each for one modality, and aligns the latent spaces. The latent space, thus, can enable information sharing among different modality sources. LisGAN \cite{li2019leveraging} is inspired by the multi-view property of images and improves f-CLSWGAN by encouraging the generated samples to approximate at least one visually representative view of samples. CANZSL \cite{chen2020canzsl} considers the cycle-consistency principle of image generation and proposes a cycle architecture by translating synthesized visual features into semantic information. ABP-ZSL \cite{zhu2019learning} adopts the rarely studied generative models ABPs to generate visual features for unseen classes. GDAN \cite{huang2019generative} incorporates a flexible metric in the model’s discriminator to measure the similarity of features from different modalities. 

The bidirectional conditional generative models enforce cycle-consistent generation and allow the generated images to truthfully reflect the conditional information \cite{zhu2017unpaired,chen2020canzsl}. Instead of encouraging cycle consistency through adding additional reverse networks, generative flows are bidirectional and cycle-consistent in nature. The generative flows are designed to infer and generate within the same network. Also, the generative flows are lightweight comparing to other methods as no auxiliary networks are needed, \textit{e.g.,} discriminator for GANs, variational encoder for VAEs. Some conditional generative flows \cite{ardizzone2018analyzing,ardizzone2019guided} are proposed to learn image generation from class-level semantic information. IZF \cite{shen2020invertible} adopts the invertible flow model \cite{ardizzone2018analyzing} for GZSL. It implicitly learns the conditional generation by inferring the semantic vectors. Such implicit encoding may cause the generated samples to be incoherent with the given attributes. Instead, we explicitly blend the semantic information into each of the coupling layers of the generative flow, learning the semantically consistent visual features. We also argue that the MMD regularization in IZF is inappropriate for GZSL, since the seen and unseen classes are coalesced. More explanation is depicted in Section 3.2.

% It enforces conditional generation by mixing the conditional vectors with the prior. However, this design weakens the conditional information through the affine coupling layers. In our framework, instead, we progressively input the conditional information in each affine coupling layer, which enhances the semantic information in the generation process.

\subsection{Visual Perturbation}
Our proposed visual perturbation approach is similar to data augmentation techniques. In many deep learning tasks, data augmentation \cite{shorten2019survey} is an effective strategy to improve model performance. Generally, bigger datasets better facilitate the learning of deep models \cite{sun2017revisiting}. Common data augmentation techniques on image data include flipping, rotating, cropping, color jittering, edge enhancement, random erasing \cite{mikolajczyk2018data}, etc. Instead of augmenting the raw data samples, DeVries and Taylor \cite{devries2017dataset} propose an augmentation strategy in the features space. In the dense feature space, the augmentation is more direct and unlimited augmented feature samples can be yielded.

Generative zero-shot learning is intrinsically a data augmentation approach to handle the zero-shot learning problem by augmenting the training data of the unseen classes. However, the augmentation power is limited by the training data of the seen classes, as the empirical distribution of training data cannot faithfully reflect the underlying real distribution of seen classes. In this case, we resort to a data augmentation strategy to complement the potential patterns depicted seen classes and further transfer to unseen classes. 

It is noteworthy that the motivation of our approach is also different from these data augmentation techniques. These methods statically augment from the real samples for training, resulting in limited augmented samples. Instead of static augmentation, our perturbation noises are sampled dynamically, leading to unlimited augmented samples. 

